Formal Verification of Stochastic Systems with ReLU Neural Network Controllers

In this work, we address the problem of formal safety verification for stochastic cyber-physical systems (CPS) equipped with ReLU neural network (NN) controllers. Our goal is to find the set of initial states from where, with a predetermined confidence, the system will not reach an unsafe configuration within a specified time horizon. Specifically, we consider discrete-time LTI systems with Gaussian noise, which we abstract by a suitable graph. Then, we formulate a Satisfiability Modulo Convex (SMC) problem to estimate upper bounds on the transition probabilities between nodes in the graph. Using this abstraction, we propose a method to compute tight bounds on the safety probabilities of nodes in this graph, despite possible over-approximations of the transition probabilities between these nodes. Additionally, using the proposed SMC formula, we devise a heuristic method to refine the abstraction of the system in order to further improve the estimated safety bounds. Finally, we corroborate the efficacy of the proposed method with simulation results considering a robot navigation example and comparison against a state-of-the-art verification scheme.

==> refer.tex <==
\begin{thebibliography}{00}
% \bibitem{b2} LeCun, Y., Bengio, Y., \& Hinton, G. (2015). Deep learning. nature, 521(7553), 436-444.

\bibitem{b3} Amini, A., Rosman, G., Karaman, S., \& Rus, D. (2019, May). Variational end-to-end navigation and localization. In 2019 International Conference on Robotics and Automation (ICRA) (pp. 8958-8964). IEEE.

\bibitem{b4} Shamsfakhr, F., \& Bigham, B. S. (2017). A neural network approach to navigation of a mobile robot and obstacle avoidance in dynamic and unknown environments. Turkish journal of electrical engineering \& computer sciences, 25(3), 1629-1642.

\bibitem{b5}Nägeli, T., Alonso-Mora, J., Domahidi, A., Rus, D., \& Hilliges, O. (2017). Real-time motion planning for aerial videography with dynamic obstacle avoidance and viewpoint optimization. IEEE Robotics and Automation Letters, 2(3), 1696-1703.

\bibitem{b6}Chen, Y. F., Everett, M., Liu, M., \& How, J. P. (2017, September). Socially aware motion planning with deep reinforcement learning. In 2017 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS) (pp. 1343-1350). IEEE.

\bibitem{b7} Schmuck, V., \& Meredith, D. (2019). Training networks separately on static and dynamic obstacles improves collision avoidance during indoor robot navigation. In European Symposium on Artificial Neural Networks, Computational Intelligence and Machine LearningEuropean Symposium on Artificial Neural Networks, Computational Intelligence and Machine Learning (pp. 655-660). Ciaco-i6doc. com. 

\bibitem{b8}Xiang, W., Musau, P., Wild, A. A., Lopez, D. M., Hamilton, N., Yang, X., ... \& Johnson, T. T. (2018). Verification for machine learning, autonomy, and neural networks survey. arXiv preprint arXiv:1810.01989.

\bibitem{b9} Charikar, M., Steinhardt, J., \& Valiant, G. (2017, June). Learning from untrusted data. In Proceedings of the 49th Annual ACM SIGACT Symposium on Theory of Computing (pp. 47-60).

\bibitem{b10} Li, B., Chen, C., Wang, W., \& Carin, L. (2019). Certified Adversarial Robustness with Additive Noise. In Advances in Neural Information Processing Systems (pp. 9459-9469).

\bibitem{b11} Fazlyab, M., Morari, M., \& Pappas, G. J. (2019). Probabilistic Verification and Reachability Analysis of Neural Networks via Semidefinite Programming. arXiv preprint arXiv:1910.04249.

\bibitem{b12} Fazlyab, M., Morari, M., \& Pappas, G. J. (2019). Safety verification and robustness analysis of neural networks via quadratic constraints and semidefinite programming. arXiv preprint arXiv:1903.01287.

\bibitem{b13} Katz, G., Barrett, C., Dill, D. L., Julian, K., \& Kochenderfer, M. J. (2017, July). Reluplex: An efficient SMT solver for verifying deep neural networks. In International Conference on Computer Aided Verification (pp. 97-117). Springer, Cham.

\bibitem{b14} Ivanov, R., Weimer, J., Alur, R., Pappas, G. J., \& Lee, I. (2019, April). Verisig: verifying safety properties of hybrid systems with neural network controllers. In Proceedings of the 22nd ACM International Conference on Hybrid Systems: Computation and Control (pp. 169-178).

\bibitem{b15} Ivanov, R., Carpenter, T. J., Weimer, J., Alur, R., Pappas, G. J., \& Lee, I. (2019). Case Study: Verifying the Safety of an Autonomous Racing Car with a Neural Network Controller. arXiv preprint arXiv:1910.11309. controllers

% \bibitem{b16} Chen, X., Ábrahám, E., \& Sankaranarayanan, S. (2013, July). Flow*: An analyzer for non-linear hybrid systems. In International Conference on Computer Aided Verification (pp. 258-263). Springer, Berlin, Heidelberg.

\bibitem{b17} Shoukry, Y., Nuzzo, P., Sangiovanni-Vincentelli, A. L., Seshia, S. A., Pappas, G. J., \& Tabuada, P. (2017, April). SMC: Satisfiability modulo convex optimization. In Proceedings of the 20th International Conference on Hybrid Systems: Computation and Control (pp. 19-28).

\bibitem{b1} Sun X, Khedr H, Shoukry Y. Formal verification of neural network controlled autonomous systems, Proceedings of the 22nd ACM International Conference on Hybrid Systems: Computation and Control. 2019: 147-156.

% \bibitem{b19} Bujorianu, M. L., Wisniewski, R., \& Boulougouris, E. (2020). Stochastic safety for Markov chains. IEEE Control Systems Letters, 5(2), 427-432.

\bibitem{b20} Lahijanian, M., Andersson, S. B., \& Belta, C. (2015). Formal verification and synthesis for discrete-time stochastic systems. IEEE Transactions on Automatic Control, 60(8), 2031-2045.

\bibitem{b21} Dutreix, M., \& Coogan, S. (2018, April). Efficient verification for stochastic mixed monotone systems. In 2018 ACM/IEEE 9th International Conference on Cyber-Physical Systems (ICCPS) (pp. 150-161). IEEE.

\bibitem{b22} Dutreix M, Coogan S. Specification-guided verification and abstraction refinement of mixed monotone stochastic systems[J]. IEEE Transactions on Automatic Control, 2020.

\bibitem{b23} Zarei, M., Wang, Y., \& Pajic, M. (2020, April). Statistical verification of learning-based cyber-physical systems. In Proceedings of the 23rd International Conference on Hybrid Systems: Computation and Control (pp. 1-7).

\bibitem{b24} Wang, Y., Zarei, M., Bonakdarpour, B., \& Pajic, M. (2019). Statistical verification of hyperproperties for cyber-physical systems. ACM Transactions on Embedded Computing Systems (TECS), 18(5s), 1-23.

\bibitem{b18} Blackmore L, Ono M, Williams B C. Chance-constrained optimal path planning with obstacles[J]. IEEE Transactions on Robotics, 2011, 27(6): 1080-1094.

\end{thebibliography}
% \vspace{12pt}
% \color{red}
% IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.


